Learning Over Dirty Data Without Cleaning

Real-world datasets are dirty and contain many errors. Examples of these issues are violations of integrity constraints, duplicates, and inconsistencies in representing data values and entities. Learning over dirty databases may result in inaccurate models. Users have to spend a great deal of time and effort to repair data errors and create a clean database for learning. Moreover, as the information required to repair these errors is not often available, there may be numerous possible clean versions for a dirty database. We propose DLearn, a novel relational learning system that learns directly over dirty databases effectively and efficiently without any preprocessing. DLearn leverages database constraints to learn accurate relational models over inconsistent and heterogeneous data. Its learned models represent patterns over all possible clean instances of the data in a usable form. Our empirical study indicates that DLearn learns accurate models over large real-world databases efficiently.

==> 5.Sampling.tex <==
\section{Efficient Learning Through Sampling}
\label{section:heterolearn-sampling}

%\subsection{Rationale for Sampling}

The set of tuples $I_{e}$ created in bottom-clause construction may be large if many tuples in $I$ are relevant to $e$.
Thus, bottom-clause $C_e$ would be very large, making the learning process extremely time-consuming.
This problem is exacerbated when using similarity search operators to find relevant tuples, as many entities have similar names.
To overcome this problem, CastorX samples from the tuples in $I_{e}$ to obtain 
a smaller tuple set $I_{e}^s \subseteq I_{e}$.

A {\it sample $I^s$ of a database} $I$ is a subset of the tuples in $I$.
The {\it inclusion probability} of tuple $t \in I$ is the probability that $t$ is included in $I^s$. 
The inclusion probabilities may differ for each tuple, according to the sampling technique.

Given clause $C$ and literal $R(\bar{u})$ in $C$, we call $\bar{u}$ that may contain both variables and constants a {\it free tuple}.
A {\it canonical database instance} of clause $C$, shown as $I^C$,
is the database instance whose tuples are the free tuples in $C$~\cite{AliceBook}. 
Given a clause $C$, we can build its canonical database instance $I^C$, and vice versa.

Consider the clause $C: T(\bar{u_0}) \leftarrow R_1(\bar{u_1}), \ldots, R_n(\bar{u_n})$.
Let $I^C$ be the canonical database instance of $C$.
We call the free tuple $\bar{u_0}$ in $I^C$ that comes from the head of $C$ the {\it seed tuple}.
Let $I^{Cs}$ be a sample of the canonical database $I^C$.
A {\it sample $C^s$ of a clause} $C$ is a clause built from $I^{Cs}$ that must satisfy the following properties:
\begin{itemize}
	\item $C^s$ contains the same head relation as $C$, i.e., $I^{Cs}$ must contain seed tuple $\bar{u_0}$.
	\item All literals in $C^s$ must be head-connected, i.e., all tuples in $I^{Cs}$ must be connected to the seed tuple by using only tuples in $I^{Cs}$.
\end{itemize}

One approach to obtain a sample $C^s$ of a bottom-clause $C$ is to first compute the full bottom-clause $C$ and then sample from it.
%This is equivalent to computing the canonical database instance $I^C$, and then sampling from it.
A more efficient approach is to sample {\it during} bottom-clause construction.
Instead of computing $C$ and then sampling from it, we directly compute $C^s$.
One way to do this is to restrict the number of literals added to the bottom-clause per relation~\cite{aleph,progolem,castor:SIGMOD17}.
This is done by sampling from the tuples in $I_R$ in Algorithm~\ref{algorithm:bottom-clause-original} (lines 7 and 9).
The parameter that restricts the maximum number of tuples in the sample of $I_R$ is called the {\it sample size}.
In the following sections, we provide concrete sampling techniques.

%-------------------------------------------------------------
%\subsection{Sampling Techniques}
%\label{section:sampling}
%For ease of explanation, we explain our sampling techniques for the case where we get as input a single database $I$. These techniques generalize to the case where we get as input multiple database instances.
%-------------------------------------------------------------
\subsection{Na\"ive Sampling}
Let $C_e$ be a bottom-clause associated with example $e$.
A {\it na\"ive sample} $C_e^s$ of clause $C_e$ is the clause obtained the following way.
Let $I_R$ be the set of tuples in relation $R$ that can be added to $I_e$ (lines 10-11 in Algorithm~\ref{algorithm:bottom-clause-original}).
We obtain a {\it uniform} sample $I_R^s$ of $I_R$ and only add tuples in $I_R^s$ to $I_e$.
In a uniform sample, every tuple in $I_R$ is sampled independently with the same inclusion probability, i.e., $\forall t \in I_R, \tau(t) = \frac{1}{|I_R|}$.
This method is used by current relational learning algorithms~\cite{progolem,castor:SIGMOD17}.


%-------------------------------------------------------------
\begin{comment}
\subsection{Commutativity of Sampled Learning and Integration}

Let {\it Sample($I$)} return a sample of $I$.
\begin{theorem}
	The set of Horn definitions learned over each stable instance in a sample of all stable instances is the same as 
	the set of Horn definitions obtained by learning over a sample of the unclean instance, and then enforcing MDs, i.e.,
%	{\it Learn(Sample(StableInstances($I, \Sigma$), $E$))} = {\it StableDefinitions(Learn(Sample($I$), $E, \Sigma$))}
	\begin{align*}
		\mathit{Learn}&(\mathit{Sample}(\mathit{StableInstances}(I, \Sigma), E)) = \\
		& \mathit{StableDefinitions}(\mathit{Learn}(\mathit{Sample}(I), E, \Sigma))
	\end{align*}
\end{theorem}
\begin{proof}
	TODO.
\end{proof}


%As mentioned in Section~\ref{}, a bottom-clause with similarity literals is a compact representation of multiple bottom-clauses.
%Because we can exchange sampling and cleaning, a bottom-clause containing similarity literals that is created by sampling from multiple (heterogeneous) databases is also a compact representation of all bottom-clauses created by sampling over all stable instances.


\end{comment}
%-------------------------------------------------------------
\subsection{Approximate Coverage Testing}
\label{section-approximate}

As mentioned in Section~\ref{sec:generalization}, CastorX uses $\theta$-subsumption to compute the coverage of candidate clauses.
Ideally, a ground bottom-clause $G_e$ for example $e$ must contain one literal per each tuple in the database that is connected to $e$ through some (similarity) joins.
Otherwise, the $\theta$-subsumption test may declare that $C$ does {\it not} cover $e$ when $C$ actually covers $e$.
However, it is expensive to check $\theta$-subsumption for large clauses.
Therefore, to improve efficiency, we apply the sampling techniques explained in the previous sections to build ground bottom-clauses.
Because we use a sampled bottom-clause $G^s_e$, checking whether $C \subseteq_{\theta} G^s_e$ is an approximation of checking whether $I \wedge C \models e$, meaning that there may be errors.
Nevertheless, our empirical results, reported in Section~\ref{section:experiments}, indicate that, with the appropriate sample size, this issue does {\it not} significantly impact the accuracy of the learned definitions. 
The learning algorithm involves many (thousands) coverage tests.
Because CastorX reuses ground bottom-clauses, it can run efficiently over large databases.



%To improve the efficiency of evaluation, we can approximately evaluate clauses by using the sampling techniques introduced in Section~\ref{section-sampling} to build ground bottom-clauses, which are then used to check coverage.


%To reduce the time of evaluation, CastorX samples $I_e$ to obtain a subset $I_e^s \in I_e$, as done in Section~\ref{section-sampling}. 
%CastorX builds $C^g_e$ based on $I_e^s$, instead of $I_e$.
%Because $I_e^s$ is a sample of $I_e$, checking whether $C \subseteq_{\theta} C^g_e$ is an approximation of checking whether $I \wedge C \models e$, meaning that there may be errors.
%A good sampling technique to obtain $I_e^s \in I_e$ reduces errors.
%%CastorX uses the sampling techniques introduced in Section~\ref{section-sampling}.
%The learning algorithm involves many (thousands) coverage tests.
%Because CastorX reuses ground bottom-clauses, it can run efficiently, even over large databases.



